Stochastic and Quantum Dynamics of Repulsive Particles: from Random Matrix Theory to Trapped Fermions

This statistical physics thesis focuses on the study of three kinds of systems which display repulsive interactions: eigenvalues of random matrices, non-crossing random walks and trapped fermions. These systems share many links, which can be exhibited not only at the level of their static version, but also at the level of their dynamical version. We present a combined analysis of these systems, employing tools of random matrix theory and stochastic calculus as well as tools of quantum mechanics, in order to solve some original problems. Further from the detailed presentation of the field and the report of the results obtained during the PhD, the different themes exposed in the chapters of the thesis allow for perspectives on related issues. As such, the first chapter is an introduction to random matrix theory; we detail its historical evolution and numerous applications, and present its essential concepts, constructions and results. The second chapter discusses non-crossing random walks; we describe the deep links they share with random matrix eigenvalue processes and showcase the results obtained in the scope of boundary problems. In the third chapter, which focuses on stochastic matrix processes, we introduce in particular a process inspired from the Kesten random recursion, and highlight the new link it allows to draw between the inverse-Wishart ensemble and fermions trapped in the Morse potential. Lastly, the fourth chapter, centred on the particular case of bridge processes, allows for a joint treatment of scalar and matrix models; therein, we develop a generalization of the Ferrari-Spohn problem for non-crossing scalar bridges and, as an opening, we exhibit the connections of matrix bridges with other aspects of random matrices.

==> bib/babelbst.tex <==
%%

%% This is file `merlin.tex',

%% generated with the docstrip utility.

%%

%% The original source files were:

%%

%% merlin.mbs  (with options: `bblbst')

%% 

%% IMPORTANT NOTICE:

%% 

%% For the copyright see the source file.

%% 

%% Any modified versions of this file must be renamed

%% with new filenames distinct from merlin.tex.

%% 

%% For distribution of the original source see the terms

%% for copying and modification in the file merlin.mbs.

%% 

%% This generated file may be distributed as long as the

%% original source files, as listed above, are part of the

%% same distribution. (The sources need not necessarily be

%% in the same archive or directory.)

%% Copyright 1994-2011 Patrick W Daly

 % ===============================================================

 % IMPORTANT NOTICE:

 % This bibliographic style (bst) file has been generated from one or

 % more master bibliographic style (mbs) files, listed above.

 %

 % This generated file can be redistributed and/or modified under the terms

 % of the LaTeX Project Public License Distributed from CTAN

 % archives in directory macros/latex/base/lppl.txt; either

 % version 1 of the License, or any later version.

 % ===============================================================

 % Name and version information of the main mbs file:

 % \ProvidesFile{merlin.mbs}[2011/11/18 4.33 (PWD, AO, DPC)]

 % This is babelbst.tex for English.

 % It should serve as a model for other languages.

 % Alternatively, store it under a different name (e.g. englbst.tex)

 % and then \input it with a command in babelbst.tex.

\def\bbland{and}                \def\bbletal{et~al.}

\def\bbleditors{editors}        \def\bbleds{eds.}

\def\bbleditor{editor}          \def\bbled{ed.}

\def\bbledby{edited by}

\def\bbledition{edition}        \def\bbledn{edn.}

\def\bblvolume{volume}          \def\bblvol{vol.}

\def\bblof{of}

\def\bblnumber{number}          \def\bblno{no.}

\def\bblin{in}

\def\bblpages{pages}            \def\bblpp{pp.}

\def\bblpage{page}              \def\bblp{p.}

\def\bbleidpp{pages}

\def\bblchapter{chapter}        \def\bblchap{chap.}

\def\bbltechreport{Technical Report}

\def\bbltechrep{Tech. Rep.}

\def\bblmthesis{Master's thesis}

\def\bblphdthesis{Ph.D. thesis}

\def\bblfirst{First}            \def\bblfirsto{1st}

\def\bblsecond{Second}          \def\bblsecondo{2nd}

\def\bblthird{Third}            \def\bblthirdo{3rd}

\def\bblfourth{Fourth}          \def\bblfourtho{4th}

\def\bblfifth{Fifth}            \def\bblfiftho{5th}

\def\bblst{st}  \def\bblnd{nd}  \def\bblrd{rd}

\def\bblth{th}

\def\bbljan{January}  \def\bblfeb{February}  \def\bblmar{March}

\def\bblapr{April}    \def\bblmay{May}       \def\bbljun{June}

\def\bbljul{July}     \def\bblaug{August}    \def\bblsep{September}

\def\bbloct{October}  \def\bblnov{November}  \def\bbldec{December}

\endinput

%%

%% End of file `merlin.tex'.


==> preamb/work.tex <==
% !TeX encoding = UTF-8
%%% préambule pour les paquets à usabe temporaires %%%
%%% Génération de fake text, et marquage des versions de travail  : à supprimer ! %%%
\usepackage{lipsum} 
\usepackage{blindtext}
\blindmathtrue
\AddToShipoutPictureBG{% Add picture to background of every page
  \AtPageLowerLeft{%
   \raisebox{3\baselineskip}{\makebox[\paperwidth][c]{Version \today, \currenttime}}%
}}
\usepackage[notref,notcite]{showkeys}
%\usepackage[pdftex]{changebar}
\usepackage{versions}          % permet d'activer ou non certains environnements

%\AfterEndPreamble{\nocite{*}}



==> sections/chap5.tex <==
\chapter{Eigenvalue statistics of random matrices and quantum transport} 
\chaptermark{RMT eigenvalue statistics and quantum transport}
\label{chap:5}

\cite{Xu2019,Anderson2019}


\section{Transport in the XX chain}
\section{Extension to a general initial condition}
\section{Transport and initial correlations}

==> sections/indextablefigures.tex <==
\chapter{List of Figures}


\begin{tabular}{p{2.5cm}  l }
Fig. \ref{fig:surmise} & Wigner's surmise\\[5pt]
Fig. \ref{fig:portraits} & \textit{John Wishart, Eugene Wigner and Freeman Dyson} \\ 
 & Sources : Wikipedia and New York Times \\[5pt]
 test & test
\end{tabular} 
 
